Response time central-limit and failure rate estimation for stationary periodic rate monotonic real-time systems

Real-time systems consist of a set of tasks, a scheduling policy, and a system architecture, all constrained by timing requirements. Many everyday embedded systems, within devices such as airplanes, cars, trains, and spatial probes, operate as real-time systems. To ensure safe failure rates, response times-the time required for the exection of a task-must be bounded. Rate Monotonic real-time systems prioritize tasks according to their arrival rate. This paper focuses on the use of the central limit of response times built in \cite{zagalo2022} and an approximation of their distribution with an inverse Gaussian mixture distribution. The distribution parameters and their associated failure rates are estimated through a suitable re-parameterization of the inverse Gaussian distribution and an adapted Expectation-Maximization algorithm. Extensive simulations demonstrate that the method is well-suited for the approximation of failure rates. We discuss the extension of such method to a chi-squared independence test adapted to real-time systems.

==> figures/runtime.tex <==
	\begin{figure}[ht]
	\centering
	\begin{tikzpicture}
		% Toutes les options de l'axe sur une seule ligne (pour éviter l'erreur)
		\begin{loglogaxis}[
			xlabel={Sample size}, 
			ylabel={Running time (ms)}, 
			xmin=5, xmax=20000, 
			ymin=0.05, ymax=30, 
			grid=major, 
			legend pos=north west,
			legend style={draw=black, fill=white}
			]
			
			% --- 1. Courbe ROUGE (dogleg) ---
			\addplot[
			color=red, 
			mark=triangle*, 
			thick
			] 
			coordinates {
				% Ordre des Y : Basse
				(10, 0.15)
				% Ordre des Y : Moyenne
				(100, 0.27)
				% Ordre des Y : Moyenne
				(1000, 1.3)
				% Ordre des Y : Basse
				(10000, 8.0)  
			};
			\addlegendentry{Powell's dog-leg}
			
			% --- 2. Courbe BLEUE (newton) ---
			\addplot[
			color=blue, 
			mark=square*, 
			thick
			] 
			coordinates {
				% Ordre des Y : Haute
				(10, 0.2)     
				% Ordre des Y : Haute
				(100, 0.35)    
				% Ordre des Y : Basse (Croisement avec Dogleg et Brent)
				(1000, 0.9)    
				% Ordre des Y : Haute
				(10000, 12.5)  
			};
			\addlegendentry{Newton-Raphson}
			
			% --- 3. Courbe VERTE (brent) ---
			\addplot[
			color=green!60!black, 
			mark=o,               
			thick
			] 
			coordinates {
				% Ordre des Y : Basse (Croisement avec Dogleg et Newton)
				(10, 0.1)     
				% Ordre des Y : Basse
				(100, 0.2)    
				% Ordre des Y : Haute
				(1000, 1.7)    
				% Ordre des Y : Moyenne
				(10000, 10.2)   
			};
			\addlegendentry{BFGS}
			
		\end{loglogaxis}
	\end{tikzpicture}
	
	\caption{Running time of the EM algorithm, using various Newton-like minimization algorithms to solve \eqref{eq:min}. %All three methods appear to be equivalent.}\label{fig:runningtime}
\end{figure}

==> hitl.tex <==
\subsection{HITL Data} \label{sec:data}

In this section we use the IG method on HITL data. Note that in this case, execution times are not necessarily independent. However, we test our method applied to real-data performs. We use a real case of 9 programs of an autopilot of a drone, \textsc{px4-rt} \cite{sorel2024kopernic,9804670,ntaryamira:tel-03789654,hawila2025period}, a modified version of \textsc{px4} \cite{7140074} with a real-time behavior, and a clock-measuring that can preempt the operating system itself. \textsc{px4-rt} is run on an ARM Cortex M4 CPU clocked at $180$ MHz with $256$ KB of RAM using a simulated environment from Gazebo \cite{koenig2004design}. \textsc{px4-rt} allows to measure execution times (Figures~\ref{fig:simtasksetpx4} and Table~\ref{tab:px4}) and response times during the flight of a drone. It runs on top of \textsc{NuttX}, a real-time operating system (RTOS). It provides an infrastructure for internal communications between all programs and off-board applications. Each task is a \textsc{NuttX} task launched at the beginning of the \textsc{px4} program. The tasks read data from sensors (\textit{snsr}), estimate positions and attitudes using a Kalman filter (\textit{ekf2}), control the position (\textit{pctl}) and the attitude (\textit{actl}) of the drone, the flight manager (\textit{fmgr}), the hover thrust estimator (\textit{hte}), command the state of the drone (\textit{cmdr}), and the rate controller (\textit{rctl}), which is the inner-most loop to control the body rates. These tasks are in constant interference with the operating system \textsc{NuttX}, which makes them statistically dependent. Because the operating system has the highest priority, the nine tasks studied are constantly preempted by \textsc{NuttX}. Unfortunately, it is not possible to get information about the operating system programs that interfere. Unlike the simulation in Section~\ref{sec:simulations}, \textsc{px4-rt} runs concurrently with other tasks which do not have timing requirements, making it a complex system with many unknown variables. We test in this section whether and when the proposed parametric estimation is suitable for such complex system.

In this case, the distribution functions of execution times cannot be provided. Therefore, we use the empirical distributions shown in \figurename~\ref{fig:simtasksetpx4}. Thus, the empirical mean utilizations $\hat{u}_i$ are computed with the empirical means of execution times, and the empirical maximal utilizations $\hat{u}^{max}_i$ with the empirical maximum of execution times. See Table~\ref{tab:px4} for a full description of the parameters. As shown in the previous section, the response times of the highest priority task \textit{snsr} are not estimated.

These programs generate response times distributions shown in \figurename~\ref{fig:droneRT_rctl}(a)-\ref{fig:droneRT_cmdr}(a), on which we use the mixture model proposed in \eqref{eq:mixture} with the EM algorithm provided in Section~\ref{sec:mle}. See \cite{9804670} for a full description of the data. The QQplots in Figures~\ref{fig:droneRT_rctl}(b)-\ref{fig:droneRT_cmdr}(b) show that the estimation is good for the large quantiles, which is what is important to determine the reliability. We can identify in \figurename~\ref{fig:droneRT_cmdr}  \figurename~\ref{fig:droneRT_navr} and \ref{fig:droneRT_fmgr} that for the \textit{cmdr}, \textit{navr} and \textit{fmgr} tasks the estimation is not good enough, which means that those programs are mutually dependent (operating system etc.), and that a feasibility test on this task would not be suitable with the method built in this paper. Nevertheless, for the other tasks the approximation is  good and can therefore be used for a feasibility analysis. 





%{figure*}[p]
%	\foreach \ii in {snsr, rctl, ekf2, actl, pctl, fmgr,hte, navr, cmdr}{%
%		\begin{subfigure}[b]{0.3\textwidth}%
%			\centering 
%%			\includegraphics[width=0.8\textwidth]{figures/\ii-eps-converted-to.pdf}
	%		\caption{Task $\ii$}
	%	\end{subfigure}
%	}%
%	\caption{Execution time empirical probability functions of the 9 studied tasks of the drone autopilot.}
%	\label{fig:simtasksetpx4}
%{figure*}

%	\begin{figure*}[p]
	%	\ContinuedFloat 
	%	\foreach \ii in {hte, navr, cmdr}{%
		%			\begin{subfigure}[b]{0.5\textwidth}%
			%				\centering 
			%				\includegraphics[width=0.8\textwidth]{figures/\ii.eps}
			%				% \label{fig:simtasksetpx4_\ii}
			%				\caption{Task $\ii$}
			%			\end{subfigure}
		%	}%
	%	\caption{Execution time empirical probability functions of the 9 studied tasks of the drone autopilot.}
	%	\end{figure*}


\input{tables/table_px4}

	\begin{figure*}[b]
		\centering
	%	\begin{subfigure}[b]{0.8\textwidth}
	%		\includegraphics[width=\textwidth]{figures/rt_\ii.pdf}
	%		\caption{Response times empirical distributions (black) and MLE distribution (red)} 
	%	\end{subfigure}
	%	\hfill
	\foreach \ii in {rctl, ekf2, actl, pctl, fmgr, hte, navr, cmdr}{%
		\begin{subfigure}[b]{0.24\textwidth}
			\includegraphics[width=\textwidth]{figures/qqplot_\ii.pdf}
		\caption{$\ii$ task of \textsc{px4-rt}} 
		\label{fig:droneRT_\ii}
		\end{subfigure} 
	}%
		\caption{QQplot with the $\chi^2_1$ quantiles from \eqref{eq:chi} where each color represents a component of the mixture. The closer to the red line the better the estimation.}

	\end{figure*}




